Dynamic Visual Reasoning by Learning Differentiable Physics Models from Video and Language

In this work, we propose a unified framework, called Visual Reasoning with Differ-entiable Physics (VRDP), that can jointly learn visual concepts and infer physics models of objects and their interactions from videos and language. This is achieved by seamlessly integrating three components: a visual perception module, a concept learner, and a differentiable physics engine. The visual perception module parses each video frame into object-centric trajectories and represents them as latent scene representations. The concept learner grounds visual concepts (e.g., color, shape, and material) from these object-centric representations based on the language, thus providing prior knowledge for the physics engine. The differentiable physics model, implemented as an impulse-based differentiable rigid-body simulator, performs differentiable physical simulation based on the grounded concepts to infer physical properties, such as mass, restitution, and velocity, by fitting the simulated trajectories into the video observations. Consequently, these learned concepts and physical models can explain what we have seen and imagine what is about to happen in future and counterfactual scenarios. Integrating differentiable physics into the dynamic reasoning framework offers several appealing benefits. More accurate dynamics prediction in learned physics models enables state-of-the-art performance on both synthetic and real-world benchmarks while still maintaining high transparency and interpretability; most notably, VRDP improves the accuracy of predictive and counterfactual questions by 4.5% and 11.5% compared to its best counterpart. VRDP is also highly data-efficient: physical parameters can be optimized from very few videos, and even a single video can be sufficient. Finally, with all physical parameters inferred, VRDP can quickly learn new concepts from a few examples.

==> supps/datatype_tab.tex <==
\begin{table}[t]
\centering
%\renewcommand{\arraystretch}{0.9}
%\setlength{\tabcolsep}{0.3em}
%\resizebox{1\linewidth}{!}{
\begin{tabular}{ll}
\toprule
Type     & Semantics \\
\midrule
\textit{object} &   A single object in the video. \\
\textit{objects}   & A set of objects in the video. \\
\textit{event}  & A single event in the video. \\
\textit{events}  & A set of events in the video. \\
\textit{order} & The chronological order of an event, \eg ``First'', ``Second'' and ``Last''. \\
%\textit{color}  & An indication of a color, including ``blue'', ``brown'', ``cyan'', ``gray'', ``green'', ``purple'' ,  ``red'' and ``yellow''. \\
%\textit{material} & An indication of a material including ``metal'' and ``rubber''. \\
%\textit{shape} & An indication of a shape including ``cube'', ``cylinder'' and ``sphere''. \\
\textit{static concept} & Object-level static concepts like ``Red'', ``Sphere'' and ``Metal''. \\
\textit{dynamic concept} & Object-level dynamic concepts like ``Moving'' and ``Stationary''. \\
\textit{attribute} & Static attributes including ``Color'', ``Shape'' and ``Material''. \\
\textit{frame}  & The frame number of an event. \\
\textit{int} & A single integer like ``0'' and ``1''. \\
\textit{bool} & A single boolean value, ``True'' or ``False''. \\
\textit{representations} & The visual features that are calculated from object trajectories. \\
\bottomrule
\end{tabular}
\caption{The data types on CLEVRER~\cite{yi2019clevrer}.}
\label{tb:datatype}
\end{table}

==> supps/neural_op_tab.tex <==
\begin{table}[htbp]
\centering
%\renewcommand{\arraystretch}{0.95}
%\setlength{\tabcolsep}{0.3em}
\resizebox{1\linewidth}{!}{
\begin{tabular}{cll}
\toprule
Type    & Operation/ Signature & Implementation\\ %Semantics  \\
\midrule
\multirow{10}{2cm}{Input Modules} 
               & \texttt{Objects}  &  $\textit{objects}=\textbf{1}$  \\  
               & $()\rightarrow~\textit{objects}$ \\
               & \texttt{Events}   &  $\textit{events}^{type}$ for $type \in \{in, out, col.\}$ \\
               &  $()\rightarrow ~\textit{events}$ \\
               & \texttt{UnseenEvents}   &   $\textit{events}^{col'}$ and $\textit{events}^{out'}$\\
               &  $()\rightarrow  \textit{events}$  \\
               %& \texttt{AllEvents}  &$()\rightarrow \textit{events}$  &  \\
               %& Returns all possible events on / between any objects & \\
               & \texttt{Start}  &  $M_t=1$ if $t<5$ else $M_t=0$ \\
               & $()\rightarrow  \textit{M}$ \\ 
               & \texttt{end}  &  $M_t=1$ if $t>(T-5)$ else $M_t=0$ \\
                & $()\rightarrow  \textit{M}$ \\
\midrule
\multirow{4}{1cm}{Object Filter Modules} 
& \texttt{Filter\_static\_concept}  & $\min(objs, \text{ObjFilter(\textit{sa})})$ \\
& $ (\text{objs:}~\textit{objects},~\text{sa:}~\textit{concept}) \rightarrow \textit{objects} $ \\
%& \texttt{Filter\_material} & $ (\textit{objects}, \textit{material}) \rightarrow \textit{objects} $  \\
%&  Selects objects from the input list with the input material & \\ 
%& \texttt{Filter\_shape} & $ (\textit{objects}, \textit{shape}) \rightarrow \textit{objects} $  \\
%&  Selects objects from the input list with the input shape & \\
& \texttt{Filter\_dynamic\_concept} & $\min(objects, \text{ObjFilter(\textit{da},t)})$\\
& $ (\text{objs:}~\textit{objects},\text{da:}~\textit{concept},\text{t:}~\textit{frame}) \rightarrow \textit{objects} $ \\
%&  Selects objects in the input frame with the dynamic concept & \\ 
%& \texttt{Filter\_stationary} & $ (\textit{objects}, \textit{frame}) \rightarrow \textit{objects} $  \\
%&  Selects all stationary objects in the input frame & \\
\midrule
\multirow{18}{1cm}{Event Filter Modules} 
& \texttt{Filter\_in} & $\min(objs, \text{events}^{in})$ \\
& $(\text{events}^{in}: \textit{events}, \text{objs:}~\textit{objects}) \rightarrow \textit{events}$ \\
& \texttt{Filter\_out} & $\min(objs, \text{events}^{out})$ \\
& $ (\text{events}^{out}:~\textit{events},\text{objs:}~\textit{objects}) \rightarrow \textit{events} $ \\
& \texttt{Filter\_collision} & $\min(objs^{exp}, \textit{events}^{col.})$  \\
& $ (\text{events}^{col}\text{:}~\textit{events}, \text{objs:}~\textit{objects}) \rightarrow \textit{events} $ \\
& \texttt{Get\_col\_partner} & $\max_{k\in[1,K]}(\text{events}^{col}_{n,k})$  \\
& $ (\text{events}^{col}: \textit{events}, obj_n:~\textit{object} ) \rightarrow \textit{objects}$ \\
& \texttt{Filter\_before}   & $events_n^{in}=-1$ if $t^{in}_n>t^{event1}$ \\
& $(events_n^{in}:~\textit{events}, \text{event1:}~\textit{event})$ \\
& \texttt{Filter\_after} & $events_n^{in}=-1$ if $t^{in}_n<t^{event1}$ \\
& $ (events_n^{in}:~\textit{events}, \text{event1:}~\textit{event}) \rightarrow \textit{events} $  \\
& \texttt{Filter\_order} &  $events_n^{in}>0$ if $order^{in}_n=or$ \\
& $ (events_n^{in}:~\textit{events}, \text{or:}~\textit{order}) \rightarrow \textit{event} $  \\
& \texttt{Filter\_ancestor} & {$ \{\text{event1}_n>0~\text{and}~\text{events1}_n$} \\
& $ (\text{event1:}~\textit{event}, \text{events1:}~\textit{events}) \rightarrow \textit{events} $ & \text{in the causal graph of} event1\} \\
& \texttt{Get\_frame} &  $t^{event1}$ \\
& $ (\text{event1:}~\textit{event}) \rightarrow \textit{frame} $  \\
%& \texttt{Get\_object} & \\
%& $ (\textit{event}) \rightarrow \textit{object} $  \\
\midrule
\multirow{14}{1cm}{Output Modules}
& \texttt{Query\_Attribute} &  $P^{op}=\frac{ObjFilter(op) \cdot i^{op}_a }{\sum_{op'}{ObjFilter(op') \cdot} i^{op'}_a }$\\
& $ (\text{obj:}~\textit{object}, \text{a:}~\textit{attribute}) \rightarrow \textit{concept}$  \\
%& \texttt{Query\_material} & $ (\textit{object}) \rightarrow \textit{material} $  \\
%& Returns the material of the input objects & \\ 
%& \texttt{Query\_shape} & $ (\textit{object}) \rightarrow \textit{shape} $  \\
%& Returns the shape of the input objects & \\ 
& \texttt{Count} & $\sum_n({\text{objs}_n}>0)$ \\
& $ (\text{objs:}~\textit{objects}) \rightarrow \textit{int} $  \\
& \texttt{Exist} & $(\sum_n({\text{objs}_n}>0))>0 $ \\
& $ (\text{objs:}~\textit{objects}) \rightarrow \textit{bool} $  \\
& \texttt{Belong\_to} & $ \text{True if event1} \in \text{events1 else False} $ \\
& $ (\text{event1:}~\textit{event}, \text{events1:}~\textit{events}) \rightarrow \textit{bool} $  \\
& \texttt{Negate} & False if bl else True \\
& $ (\text{bl:}~\textit{bool}) \rightarrow \textit{bool} $  \\
%\midrule
%& \texttt{Unique} & $argmax(objs)$ \\
%&$ (\text{objs:}~\textit{objects}) \rightarrow \textit{object} $    \\
\bottomrule
\end{tabular}
}
\caption{Neural operations in \alias. $\textit{events}^{col'}$ denotes the \textit{collision} events happening at the unseen future frames. $\textit{objs}^{exp} \in \mathbb{R}^{N \times N \times K}$ and $\textit{objs}^{exp}_{n_1, n_2, k}=\max(objs_{n_1}, objs_{n_2})$. $events_{n, k}^{col}$ denotes all the collision events that the $n$-th object get involved at the $k$-th frame.}
\label{tb:neural_op}
\end{table}

==> tables/algorithm.tex <==
% \begin{wrapfigure}{r}{0.7\linewidth}
% \vspace{-20pt}
\begin{figure}[t]
% \begin{minipage}[t]{0.6\linewidth}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=\linewidth]{figures/illustration.pdf}
%     \caption{.}
%     \label{fig:illustration}
% \end{figure}
% \end{minipage}
% \hfill
\centering
\begin{minipage}[t]{\linewidth}
\begin{algorithm}[H]
% \begin{small}
\caption{The learning process of differentiable physical parameters.}
\begin{algorithmic}[t]
\label{alg:algorithm}
\STATE {\bfseries Input:} The perceptual grounded object shapes and trajectories $L^\text{BEV}$,
\\ \qquad~~~~A rigid body dynamics engine with initialized parameters.
\STATE {\bfseries Output:} Physical parameters $R, \lambda_1, \lambda_2, \lambda_3, m, r, \alpha_0, \overrightarrow{v_0}, \overrightarrow{l_0}$.
\FOR{each iteration}
\FOR{each time step}
\STATE 1. Run differentiable simulation based on Eq.~\ref{eq:resistance} and Eq.~\ref{eq:dynamics} and update the object state;
\ENDFOR
\STATE 2. Get simulated trajectory $L'$ and compute loss $\|L' - L^\text{BEV}\|^2_2$;
\STATE 3. Backward the loss and update all physical parameters.
\ENDFOR
\STATE 4. Learning radius $R$, resistance coefficient $\lambda$ from 20 videos;
\STATE 5. Learning each object's initial state $\alpha_0, \overrightarrow{v_0}, \overrightarrow{l_0}$ from the frames before the collision in a video;
\STATE 6. Learning mass $m$ and restitution $r$ for each object by multiple steps;
\STATE 7. Re-optimize all parameters based on the last 20 frames for the predictive simulation.
\end{algorithmic}
% \end{small}
\end{algorithm}
\end{minipage}
\vspace{-10pt}
\end{figure}
% \end{wrapfigure}

